3D sans 3D Scans: Scalable Pre-training from Video-Generated Point Clouds

Despite recent progress in 3D self-supervised learning, collecting large-scale 3D scene scans remains expensive and labor-intensive. In this work, we investigate whether 3D representations can be learned from unlabeled videos recorded without any real 3D sensors. We present Laplacian-Aware Multi-level 3D Clustering with Sinkhorn-Knopp (LAM3C), a self-supervised framework that learns from video-generated point clouds reconstructed from unlabeled videos. We first introduce RoomTours, a video-generated point cloud dataset constructed by collecting room-walkthrough videos from the web (e.g., real-estate tours) and generating 49,219 scenes using an off-the-shelf feed-forward reconstruction model. We also propose a noise-regularized loss that stabilizes representation learning by enforcing local geometric smoothness and ensuring feature stability under noisy point clouds. Remarkably, without using any real 3D scans, LAM3C achieves better performance than previous self-supervised methods on indoor semantic and instance segmentation. These results suggest that unlabeled videos represent an abundant source of data for 3D self-supervised learning. Our source code is available at https://ryosuke-yamada.github.io/lam3c/.

==> sec/5_discussion.tex <==
\section{Discussion}
Our findings show that high-fidelity 3D scans are not a prerequisite for effective 3D-SSL. Despite being noisy, incomplete, and inconsistent, VGPC reconstructed from unlabeled videos prove sufficient for 3D-SSL. Perhaps most notably, \method{} performs strongly in linear probing, a setting that has not been widely explored in previous 3D-SSL methods. This indicates that these imperfect reconstructions still encode rich geometric cues relevant to real-world tasks. Overall, our results highlight a promising direction toward scalable 3D data generation. Instead of costly real 3D scans, unlabeled videos offer a far more scalable source of 3D supervision, where the key is learning to handle noisy and missing regions effectively.
